Mai Ho'om\=auna i ka 'Ai: Language Models Improve Automatic Speech Recognition in Hawaiian

In this paper we address the challenge of improving Automatic Speech Recognition (ASR) for a low-resource language, Hawaiian, by incorporating large amounts of independent text data into an ASR foundation model, Whisper. To do this, we train an external language model (LM) on ~1.5M words of Hawaiian text. We then use the LM to rescore Whisper and compute word error rates (WERs) on a manually curated test set of labeled Hawaiian data. As a baseline, we use Whisper without an external LM. Experimental results reveal a small but significant improvement in WER when ASR outputs are rescored with a Hawaiian LM. The results support leveraging all available data in the development of ASR systems for underrepresented languages.

==> figs/pseudocode.tex <==
\begin{algorithm}
\caption{\textsc{GetLogStringProb}($\text{string}$)}
\begin{algorithmic}[1]
\State $\text{string} \gets \textsc{Concat}(\text{sos\_token}, \text{string})$
\State $\text{log\_string\_prob} \gets 0$
\State $\text{h} \gets \textsc{InitHiddenState()}$ %
\For{$i = 1$ \textbf{to} $\textsc{len}(\text{string}) - 1$}
    \State $\text{next\_char\_log\_probs}, \text{h} \gets \textsc{PredictLM}(\text{string}[i], \text{h})$ %
    \State $\text{next\_char\_idx} \gets \textsc{GetIndex}(\text{string}[i+1])$
    \State $\text{log\_char\_prob} \gets \text{next\_char\_log\_probs}[\text{next\_char\_idx}]$
    \State $\text{log\_string\_prob} \gets \text{log\_string\_prob} + \text{log\_char\_prob}$
 \EndFor
\State \textbf{return} $\text{log\_string\_prob}$
\end{algorithmic}
\end{algorithm}








==> tables/data_wc.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|rrr}
\hline
\textbf{}       & \textbf{Words} & \textbf{Characters} & \textbf{Duration (seconds)} \\ \hline
Median          & 13             & 60                  & 5.16                        \\ 
Min             & 1              & 5                   & 0.69                        \\
Max             & 69             & 326                 & 26.59                       \\
Total           & 1120           & 5173                & 455.34                      \\
\hline
\end{tabular}
\caption{Summary of Words, Characters, and Audio Durations in 57 Test Data Examples}
\label{table:words_characters_durations}
\end{table}

